Gaussian Function On Response Surface Estimation

We propose a new framework for 2-D interpreting (features and samples) black-box machine learning models via a metamodeling technique, by which we study the output and input relationships of the underlying machine learning model. The metamodel can be estimated from data generated via a trained complex model by running the computer experiment on samples of data in the region of interest. We utilize a Gaussian process as a surrogate to capture the response surface of a complex model, in which we incorporate two parts in the process: interpolated values that are modeled by a stationary Gaussian process Z governed by a prior covariance function, and a mean function mu that captures the known trends in the underlying model. The optimization procedure for the variable importance parameter theta is to maximize the likelihood function. This theta corresponds to the correlation of individual variables with the target response. There is no need for any pre-assumed models since it depends on empirical observations. Experiments demonstrate the potential of the interpretable model through quantitative assessment of the predicted samples.

==> tex/2-related.tex <==
Until recently, most work on interpretable machine learning models focused on feature importance estimation.
\cite{adadi2018peeking} reviewed a wide range of methods used for explainable artificial intelligence (XAI), and the paper categorized the techniques into six groups where each technique can cover some groups.
Although the authors have not presented metamodeling as a separate technique in their work, metamodeling can be grouped by ``surrogate'' or ``model distillation'' where the paper reviewed them well.
The work has been published under the assumption that LIME (which is based on linear regression), model distillation, surrogate'' models and decision trees should be considered individually, while their functionalities are quite similar to each other in that all the techniques can explain the black-box by another understandable model.
This class of models that turn black-box into white-box using another simpler model is the main motivation of this work to group them into a general group called ``metamodels''.
This encourages a unified definition and a clearer connection between simpler models, and leads to incorporate more range of interpretable models.

\subsection{Surrogate Models}
Perhaps the most recent relevant work is Symbolic Metamodeling \cite{alaa2019demystifying}, introducing a metamodeling process by recovering a symbolic metamodel $g\in \mathcal{G}$, where $\mathcal{G}$ is a class of transparent functions, which approximates a black-box $f$ by optimizing the metamodeling loss $\ell(.)$ between $f$ and $g$, namely as:
\[
g^* = arg\min_{g\in \mathcal{G}} \ell (g,f)=||f-g||^2_2 = \int_\mathcal{X}(g(\mathbf{x})-f(\mathbf{x}))^2 dx.
\]

Some group of interpretable methods are studied under sensitivity analysis.
In this family of models, perhaps the most successful ones are LIME \cite{ribeiro2016should}, which focuses on the predictions of the underlying complex models to explain individual predictions.
LIME provides explanation by assuming that the relationships between variables in a complex model can be estimated linearly.
This encourages LIME use weighted OLS, and the following equation should be calibrated to generate an explanation:

\begin{footnotesize}\begin{eqnarray*}
&\xi(y)& = arg\min_\beta \left\{\sum_{i=1}^N exp(-\frac{D(y,z)^2}{\sigma^2}) (f(z_i)-\beta z'_i)^2 + \Omega(g) \right\},\\
&\Omega(g)& = \infty \bm{1}_{\{||\beta||_0 > K\}} \equiv 
\begin{cases}
  \infty, & \text{if }||\beta||_0>K\\    
  0, & \text{if }||\beta||_0\le K   
\end{cases}
\end{eqnarray*}
\end{footnotesize}

\noindent where $\Omega(g)$ is a regularization term that measures the complexity of the explanation $g \in G$, and $||\beta||_0$ denotes the number of non-zero coefficients of $\beta$. 
The parameter $K$ determines the explanation task, specifies what number of variables should be reported to the user.
This equation should be approximated by selecting a subset of $K$ features using a feature selection technique and then estimating the coefficients via weighted least squares.
\subsection{Shapeley Explanations}
SHAP \cite{lundberg2017unified}, which enables game theory to connect to local explanations, where each feature value of the instance is a ``player'' in a game, and the values are computed as follow:
\begin{eqnarray*}
\phi_i=\sum_{S\subseteq F \backslash \{i\}} \frac{|S|!(|F|-|S|-1)!}{|F|!} [f_{S\cup \{i\}}(x_{S\cup \{i\}}) - f_S(x_S)]
\end{eqnarray*}
where $S$ is a subset of the features used in the model, $i$ is the vector of feature values of the instance to be explained and $F$ is the set of all features.
Such models generally perturb the input slightly and measure the variations in prediction.
If the change in prediction occurred by tweaking the inputs is negligible, then the model would consider it as an unimportant variable.
This model is difficult even to approximate for curvature of response $y$, and the key limitation is that it is exponentially expensive due to the plethora of evaluations they make to quantify a model's sensitivity.
Another group, which seems to be straightforward for interpretation, is to employ a subset of methods that are inherently interpretable.
Although they are convenient to use, typically they are not complex enough to achieve the state-of-the-art performance, so they degrade the accuracy to some degree.
Linear regression, regression trees and RuleFit algorithms \cite{friedman2008predictive} are examples of interpretable models, however, many other transparent algorithms are constantly growing for this purpose.

\subsection{Neural Network Models}
Integrated Gradients \cite{sundararajan2017axiomatic}, Simple Gradients \cite{simonyan2013deep}, DeepLIFT \cite{shrikumar2017learning} and DeepSHAP \cite{fernando2019study} are examples of machine learning interpretation for gradient based models.
Among which, DeepLIFT relies on the assumption that what matters in a neural network model is not the gradient, which examines the change of $y$ as $x$ varies at a given point $x$, but the slope, which can measure the change of $y$ as $x$ differs from the baseline.
It is worth noting that slope is slightly different from gradient in that the term \textit{slope} is generally used for two variables. 
Thus, slope is the special case of the gradient operator acting on a single dimensional function, and it is the actual tangent to the curve of the function.
If we consider the slope instead of the gradient, then we can redefine the importance of a feature.
% \[
% x_i\times \frac{\partial Y}{\partial x_i} \rightarrow (x_i - x_i^{baseline})\times \frac{Y-Y^{baseline}}{x_i-x^{baseline}}
% \]
As such, neural networks and their variants are proper candidates to be explained by these methods, since the gradient can be used to explain the outcome of a neural network.
Due to the gradients approximation in their estimation pipelines, they are relatively fast in computation.

\subsection{Layer-wise Relevance Propagation}
Previously proposed work have also taken the approach of including and excluding one or more groups of input variables to measure the model's outcome.
These approaches are commonly used in computer vision applications, where the deep neural networks take the center stage \cite{simonyan2013deep, springenberg2014striving, zeiler2014visualizing, lundberg2017unified}.
These methods are somehow similar to gradient-based techniques in that they analyse the effects of being present and absent parts of the regions which the model representation is mostly responsive to, resulting in highlighting that important region.
Most work in this research domain are converged into the ability to evaluate contribution of each input variable to the target of a predictive model.
This has encouraged researchers to develop specific interpretability methods that target each neuron in a given layer to the outcome of the model \cite{leino2018influence}, and motivated further research to focus on the contribution of each input variable on the activation of a particular hidden unit (neuron conductance) \cite{conductance}.

\subsection{Other Techniques}
Some other work have used the general concept of global explanation by setting some ``rules'' on training points \cite{ribeiro2018anchors, plumb2018model}, so the interpretation is run through example-based explanations.
This family of explanations is considered, to some extent, as model-agnostic.
The example-based models explain an underlying model through instance selection rather than feature selection of a dataset.
Each training point is weighted based on the level of impact they have on the prediction, and this relationship is evaluated by an influence function.

Certain techniques utilize the idea of ``counterfactual explanations'' \cite{van2019interpretable} and ''adversarial examples'' \cite{su2019one, biggio2018wild}.
The example-based models are applicable for image and text explanation, but tabular data remains challenging. 

\subsection{Our Contribution}
This work, Gaussian Function On Response Surface Estimation or ``G-forse'', differs from previous work in four important ways: 
1) in this technique, the relationships between explanatory variables and one or more response variables are explored by studying the curvature of the underlying model via optimizing a metamodel. 
Spatial covariance functions can guarantee improvement of non-standard metrics of model approximation.
We will further discuss this.
2) The nature of explanation is different.
In interpretable models, a several transparent algorithms are available to predict outcome.
In model-agnostic methods, practitioners perturb the input variables to measure the change of outcome.
In G-forse, we approximate the original complex model by sampling points from underlying model under Gaussian process assumption.
3) The specification of measuring the level of impact is different.
Example-based explanation is described as generating explanations by fitting Random Forrest, yet another black-box model, to identify whether a variable with a zero coefficient contains global effects. Metamodeling is based upon maximizing the likelihood function rather than a randomized process, and have a correlation function that a vector of parameters corresponding to each feature seeks to maximize to identify the global explanation of the original model.
4) Metamodeling is an interpolation technique by which the unknown values are estimated through a Gaussian process controlled by a pre-defined correlation function. 
This property enables G-forse to avoid non-existence of maximum likelihood estimates as a result of Hauck-Donner effect encountered in classical GLM such as Logistic Regression \cite{morris1990statistical,venables2013modern}. This phenomenon occurs when the fitted probabilities are extremely close to zero or one.






==> tex/4-results.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The parameter $p$ controls the smooth correlation with a continuous gradient evaluated on a distance between points (i.e. $|x_j^{(i)}-x_j|$).
We expect variables with a high correlation tend to yield $e^{(-|x_j^{(i)}-x_j|^{p})}\rightarrow 1$ since $|x_j^{(i)}-x_j| \rightarrow 0$, so $Y(\bm{x}_j^{(i)})=Y(\bm{x}_j)$, and $e^{(-|x_j^{(i)}-x_j|^{p})}\rightarrow 0$ implies zero correlation because $|x_j^{(i)}-x_j| \gg 1$.
Figure \ref{fig:p} shows four different correlations settings for $p=0.1$, $0.5$, $1$ and $2$.
It is shown that the correlation trend is affected by the smoothness parameter $p$.
By decreasing $p$, the correlation drops significantly as $|x_j^{(i)}-x_j|$ reaches to $1$.
On the other hand, as $|x_j^{(i)}-x_j|$ increases than $1$, $p<1$ encourages the correlation to decay gradually, while there is a rapid decrease in the correlation effect for $p\geq 1$.
This sudden drop encourages a saturation effect, where $p=0.1$ leads the correlations to break the interpolation between $Y(\bm{x}_j^{(i)})$ and $Y(\bm{x}_j)$.
Hence, a smooth kernel ($p=2$) is appropriate for fitting smooth functions, while a non-differentiable
kernel ($p=1$) may be a better choice for fitting nondifferentiable functions \cite{bindel2018numerics}.
Figure \ref{fig:theta} presents the relationship between the $\theta_j$ and the correlation.
As it is shown, a sample point can extend its effect by varying a width parameter $\theta$.
A low value of $\theta_j$ indicates a high correlation between data points, whereas a high $\theta_j$ shows a significant contribution across the $Y(x_j)$'s $\theta_j$.
For example, if one examines an underlying model where they measure the income of an individual for varying hairstyle ($x_1$), office location ($x_2$) and age ($x_3$), we would hypothetically expect to see $\theta_1=0$, since hairstyle has no impact on income, a slightly higher value of $\theta_2$, since office location would affect the cost of living, and $\theta_3$ would be highest since age is most correlated with income.
The parameters $\theta_j$, for $j=1,\ldots,d$ can be interpreted as increasing $\theta_i$ makes the correlations drop to zero between data points.
We can then rewrite equation 3 as:
\begin{eqnarray}
K(h;\theta) &=& cor[Y(\bm{x}^{(j)}),Y(\bm{x}^{(l)})]\\ \nonumber
&\approx& exp(-\sum_{i=1}^k\theta_i|\bm{x}_i^{(j)}-\bm{x}_i^{(l)}|^2)
\end{eqnarray}
By investigating the parameter of $\theta$ for an anisotropic basis function, we can determine the order of importance of variables in a complex model.
Generally speaking, a smaller $\theta$ means that the learned function varies less in that direction, which it encourages that feature to be irrelevant for the learned function (Figure \ref{fig:thetaxy}).
\begin{figure*}[!ht]
\centering
\includegraphics[width=\textwidth]{plots/thetaxy.png}
\caption{$\theta$ parameter determines how relevant a variable is for learning a function. Larger $\theta$ means more relevant.}
\label{fig:thetaxy}
\end{figure*}
%==================
% p and theta
%==================
\begin{figure*}
       \centering
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[width=\textwidth]{plots/theta.png}
\caption{Correlations with varying $\theta$.}\label{fig:theta}
\end{subfigure}
%
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[width=\textwidth]{plots/p.png}
\caption{Correlations with varying $p$.}\label{fig:p}
\end{subfigure}
    \end{figure*}



